Mitigating Frequency Bias and Anisotropy in Language Model Pre-Training with Syntactic Smoothing

Language models strongly rely on frequency information because they maximize the likelihood of tokens during pre-training. As a consequence, language models tend to not generalize well to tokens that are seldom seen during training. Moreover, maximum likelihood training has been discovered to give rise to anisotropy: representations of tokens in a model tend to cluster tightly in a high-dimensional cone, rather than spreading out over their representational capacity. Our work introduces a method for quantifying the frequency bias of a language model by assessing sentence-level perplexity with respect to token-level frequency. We then present a method for reducing the frequency bias of a language model by inducing a syntactic prior over token representations during pre-training. Our Syntactic Smoothing method adjusts the maximum likelihood objective function to distribute the learning signal to syntactically similar tokens. This approach results in better performance on infrequent English tokens and a decrease in anisotropy. We empirically show that the degree of anisotropy in a model correlates with its frequency bias.

==> archive/analytical_proof.tex <==

% \section{POS Smoothing Gradient Signal}
% \label{section:analytic-pos-grad-signal}

% To understand why the POS Smoothing technique is successful at removing frequency bias it helps to analyze how the POS Smoothing objective changes the back-propagation gradient update steps of word embeddings. One of the decisions that must be made in language modeling is whether to tie the input word embedding and output projection matrices. In recent years, common practice has become to tie the two because of both practical memory savings and theoretical findings that doing so provides a regularization method on word embeddings \citep{inan2017tying, press2017using}. The choice of tied versus untied output matrices, however, has a considerable effect on the gradient update steps for the word embeddings \citep{press2017using}. 

% Let us analyze the gradient update step for the tied word embedding setting. The standard masked modeling loss function for a token at position $p$ in an input sequence of length $S$ is defined as $$ \mathcal{L}_p = - y_p\log(\hat{y_p}),$$ where $y_p$ represents the true output distribution for the masked token, and $\hat{y_p} = p_\theta(y|x_{i=1:S, i\ne p})$ represents the model's predicted probability.

% Let us next define some terms. We define the embedding matrix as a matrix $W \in \mathbb{R}^{|V|, S}$, where $|V|$ represents the size of the vocabulary and $S$ represents the maximum sequence length. We also define the output of the $N^{th}$ final attention block of a transformer as $H_N \in \mathbb{R}^{S, h_{emb}}$, with $h_{emb}$ as the hidden embedding dimension. Let $h_p$ represent the $p^{th}$ row of $H_N$, and $W_i$ the $i^{th}$ row of W. Classically, transformers compute $$ \hat{y_p}_i  = \sigma(h_p^TW_i) = \frac{e^{h_p^TW_i}}{\sum_{j \in |V|} e^{h_p^TW_j}}.$$ 

% We then find that $\frac{\partial \mathcal{L}_p}{\partial W_i}$ can be expressed as the sum of two terms:
% \begin{equation}
%     \frac{\partial \mathcal{L}_p}{\partial W_i} = \big(\sigma(h_p^TW_i) - y_p \big) h_p + \frac{\partial h_p}{\partial W_i}
% \label{eq:gen-grad-update}
% \end{equation}

% Notice that if the embedding and projection matrices are not tied, the first term of the previous equation is replaced with:
% \begin{equation}
%     \frac{\partial \mathcal{L}_p}{\partial W_i} = \frac{\partial \mathcal{L}_p}{\partial h_p}  + \frac{\partial h_p}{\partial W_i}
% \label{eq:gen-grad-update_untied}
% \end{equation}

% Typically $y_p$, the true distribution over the correct tokens, is modeled as a point distribution (with all probability mass placed on the single masked token). Notice that equation \cref{eq:gen-grad-update} implies that when using tied-weights, the representation for token $i$, $W_i$, is updated either towards (when $h_p^TW_i < y_p$) or away (when $h_p^TW_i > y_p$) from $h_p$. 

% Now consider what occurs for a token that is rarely observed during training and when using masked language modeling. By definition, $h_p^TW_i > y_p$ will nearly always be the case and thus at every update step the representation for that token will be moved in a direction away from $h_p$. At the limit, this leads to rare words being pushed far away in semantic space from all other frequently occurring tokens. This exact phenomenon has been described by \citeauthor{gao2018representation} as representation degeneration.  

% POS Smoothing can be thought of as a method to ensure that rare words are pushed away less from and towards other tokens that serve similar syntactic functions, in the process solving the aforementioned representation degeneration problem and instead inducing a syntactic bias in the token representations. 

==> archive/archive.tex <==

% Introduction NOTES 

Taking a closer look at the phenomenon using diagnostic analyses of minimal pairs: 
Memorization vs generalization, reliance on shortcuts, generally worse generalization skills compared to humans, lack of self-consistency (not sure this last point is relevant) 

References for the problem: Tal Linzen's work, Jasmijn Bastings's work on shortcuts, Adina Williams, Dieuwke Hupkes, Gulordava, everything around BLiMP (Alex Warstadt), elangovan-etal-2021-memorization, https://arxiv.org/abs/2202.07646, https://proceedings.neurips.cc/paper/2020/file/1e14bfe2714193e7af5abc64ecbd6b46-Paper.pdf, https://aclanthology.org/2022.acl-long.434.pdf [this one makes the point that memorization is important for generalization], https://aclanthology.org/2023.eacl-main.19.pdf [the introduction of this one gives a good summary of related work on memorization]

We show that low performance on BLiMP is coupled with preference for high-frequency words.  generalization capabilities of models (as measured by BLiMP) suffer from over-reliance on frequency effects. ... the language models have suboptimal strategies.   

What we think is the root of the problem: 
backpropagation signal for low-frequency words is too weak during training (not enough observations)
this problem becomes particularly prominent in models trained on smaller datasets. I am not yet sure where exactly we should mention this point but it is important to bring it up together with the typical arguments for smaller models (sustainability, democratization of access, cognitive plausibility). That way, we don't have to explain later why we use this particular setup with respect to training datas, vocab size, model setup

Our idea: 
abstracting from surface form of a word and focusing on its function in context. Assumption: words with similar word class distribution fulfill similar roles in context (here we need a good example, e.g.  low-frequency adjectives vs high-frequency adjectives)
Realization: smoothing backpropagation signal over words with similar word class profiles (it might be an idea to coin good terms for both the word profile and the method)

In this paper we introduce the idea of \textbf{pos-merge}, a model-agnostic and tokenization-agonstic approach for learning rare subwords via biasing the objective function to learn both standard language modeling and part of speech information. 

Results: 
Our adaption improves generalization capabilities (on BLIMP) without affecting perplexity and finetuning capabilities.
This improvement can be directly traced back to the improved representation of low-frequency words



OLD introduction: 
Representation of words is a difficult but key component of language modeling. Not only does the model's output depend on the representation, but also you need to be careful about how much learning signals the different representations receive over the course of training. Subword tokenization approaches, such as Unigram \cite, BBPE and SentencePiece are the default across a variety of  large language model architecture families, such as autoregressive GPT models (BPE), encoder-decoder T5 models, and decoder only models (RoBERTa). Subword tokens are important because they fundamentally reduce the problems of out-of-distribution words and also can learn to encode morphological structure.

==> archive/old_intro.tex <==
Representation of words is a difficult but key component of language modeling. Not only does the model's output depend on the representation, but also you need to be careful about how much learning signals the different representations receive over the course of training. Subword tokenization approaches, such as Unigram, BBPE and SentencePiece are the default across a variety of  large language model architecture families, such as autoregressive GPT models (BPE), encoder-decoder T5 models, and decoder only models (RoBERTa). Subword tokens are important because they fundamentally reduce the problems of out-of-distribution words and also can learn to encode morphological structure. In the human brain, psycho-linguistic research indicates that humans represent phonological units of meaning that are akin to the use of subwords in large language models. 

In the human brain we do not know exactly what the learning signal is that children use to learn neural subnetworks that map to some morphological units of meaning. We do know that the human brain has some prior which enables it to quickly generalize previous knowledge to unseen morphemes. We hypothesis that part of what enables this sort of behavior is the use of a prior that is implicitly encoded in the loss function that guides human language learning. We attempt to re-implement this sort of prior by forcing the loss function to also force the model to learn part of speech information. 

In this paper we introduce the idea of \textbf{pos-merge}, a model-agnostic and tokenization-agonstic approach for learning rare subwords via biasing the objective function to learn both standard language modeling and part of speech information. 

%Using a diagnostic analysis of minimal pairs and a small-data training scenario, we show that language models are over-reliant on frequency effects. We provide a method for modulating this preference by using part-of-speech distributions of subword tokens to improve the representation of rarer tokens that share the same distribution. Not only does this method reduce the frequency bias effect, but overall grammatical ability also improves... 



==> archive/old_related_lit.tex <==
Current approaches to language modeling rely on the memorization of infrequent tokens to perform well on generalization tasks \citep{feldman2020does}. However, models trained as likelihood maximizers tend to yield degenerate representations for rare tokens \citep{gao2018representation}. At each update step, rare tokens are pushed in the negative direction of most hidden states and thus infrequent tokens end up clustering together regardless of their semantics or syntactic roles. This clustering phenomenon is what explains the anisotropy of language models; rather than occupying a large manifold of the representational space, token representations lie along a narrow manifold \citep{gao2018representation, ethayarajh2019contextual}. 

\subsection{Anisotropy}

Anisotropy is usually measured by its inverse isotropy. \citeauthor{arora2016latent} and \citeauthor{mu2018all} define isotropy as:

\begin{equation}
    I(v(\cdot)) \coloneq \frac{\min_{\norm{c}=1} Z(c)}{\max_{\norm{c}=1} Z(c)}
\end{equation}
where $Z(c)$ is defined as the partition function over all tokens $w$ in the vocabulary $V$, with representations $v(w)$:
$$
    Z(c) = \sum_{w \in V} \exp(c^Tv(w))
$$
In practice, this definition of isotropy is analytically infeasible to solve; \citeauthor{ethayarajh2019contextual} instead provides a strong, and easy to implement empirical approximation for isotropy: 
\begin{equation}
\label{eq:empirical-isotropy}
    I(v(\cdot)) \coloneq \mathbb{E}_{i\ne j}\big(1-\cos(v(w_i), v(w_j))\big)
\end{equation}
Here, $w_i$ and $w_j$ are two tokens sampled from the vocabulary, and $\cos$ is defined as taking the cosine similarity of the two word representations for $w_i$ and $w_j$. In this paper we adopt this empirical definition of isotropy, and define anisotropy as simply $1-I(v(\cdot))$. 

% $$\cos(v(w_i), v(w_j)) = \frac{v(w_i)^Tv(w_j)}{\norm{v(w_i)}\norm{v(w_j)}}$$ 

\paragraph{Consequences of Anisotropy}
The extent to which anisotropy harms a model's language understanding abilities remains unclear. Some work has indicated that decreases in a model's anisotropy results in better performance on non-contextual benchmarks \citep{bis-etal-2021-much}, sentence comparison tasks \citep{su2021whitening}, and multi-lingual benchmarks \citep{rajaee2022isotropy}. In contrast, other efforts demonstrate the opposite: \citeauthor{ait2023anisotropy} find that some models with higher anisotropy improve on semantic clustering tasks, while \citeauthor{ding2022isotropy}~determine that models with less anisotropy do not perform better on common Natural Language Understanding (NLU) tasks. In fact, even the existence of anisotropy and its relationship to maximum likelihood training has recently been questioned. \citeauthor{cai2020isotropy}~find that  isotropy does exist in local manifolds of contextual word representations, and \citeauthor{godey2024anisotropy}~argue that anisotropy arises not as a result of maximum likelihood training, but rather through the learning dynamics of the Query and Key attention matrices in transformer models.

%as a consequence of the directional drift of the Q and K matrices in transformer models. 

Our paper adds nuance to this debate by introducing a new angle to study anisotropy: as an indirect measure of the extent to which a model relies on memorized token frequency effects rather than linguistic information when making predictions. 

\subsection{Improving Generalization}

%when the number of weights surpasses the number of training samples
Recent analytical work has shown that certain layers of transformer models implicitly store memorized long-tail data \citep{haviv-etal-2023-understanding, kobayashi2023transformer}. \citet{feldman2020neural} demonstrate that models memorize atypical examples to achieve the highest accuracy on long-tailed data samples. This memorization hack, however, has only been shown to work well with over-parameterized models \citep{belkin2019reconciling}. These findings suggest that with the current limited training objectives, generalization can only be achieved by large models trained on noisy datasets with sufficient long-tail samples \citep{Zheng2022AnES}. A parallel area of research has proposed that generalization might be possible by training models with inductive priors that encourage linguistic acquisition. 

\paragraph{Integrating Linguistic Information}
Several approaches have explored the integration of morphological and orthographic information in word embeddings to strengthen linguistic generalization of language models \citep{salle-villavicencio-2018-incorporating, vulic-etal-2017-morph, cotterell-schutze-2015-morphological, bhatia-etal-2016-morphological, both-blunsom-compositional-morphology}. Others have proposed syntactically-motivated objective functions, such as predicting constituency labels \citep{wang2023language}, hypernyms \citep{bai-etal-2022-better}, dependency tags \citep{cui2022lert} and POS tags \citep{martinez-etal-2023-climb} to implicitly encode syntactic information in word representations. Some approaches have even shown promising results on rare word performance by constructing token embeddings that take into account a word's surface form and surrounding context \citep{schick2019attentive,schick2020rare}. These methods all influence the representation of contextual tokens, but their effect on anisotropy remains an open question.
%In order to improve the representation of rare tokens in smaller models, a promising direction

\paragraph{Reducing Anisotropy}
Existing methods to reduce anisotropy broadly fall into three categories. The first group of approaches transforms the hidden states of language models to remove semantically uninformative directions and to preserve the dimensions of maximal isotropy \citep{arora2016simple,mu2018all, raunak2019effective,su2021whitening,bis-etal-2021-much}. The motivation for this style of intervention is that the top singular dimensions of pre-trained word representations encode frequency statistics rather than semantic or lexical information \citep{mu2018all}. The second category of methods introduce novel training objectives and regularization terms that reduce the effects of anisotropy \citep{gong2018frage,gao2018representation,wang2019improving}. This type of approach places an inductive bias on representations that pushes the embeddings of frequent and infrequent words to occupy a similar semantic space. The third set of approaches explore different training paradigms to directly minimize anisotropy, such as using normalizing flow models \citep{li2020sentence} or manipulating the gradients used in maximum likelihood models \citep{yu2022rare}.

% to the maximum likelihood training objectiv
%\citet{gong2018frage} introduce an adversarial training objective to push the embeddings of frequent and infrequent words to occupy a similar semantic space. \citet{gao2018representation} proposes a novel regularization term to the standard log-likelihood objective to better distribute the representation of rare words in semantic space. \citet{wang2019improving} guide the singular distributions of learned word representations towards isotropic pre-defined prior distributions.

\vspace{1em}
\noindent In our paper, we propose a new method for improving the representation of infrequent tokens by integrating linguistic information, and we study its effects on anisotropy. This method aims to increase generalization without needing to scale up the model or data.
In the following section, we first define a metric for quantifying the degree to which a model's word representations store linguistic information versus frequency statistics. Later, we apply this metric to our proposed methodology, and find that it correlates with anisotropy. 


==> archive/old_sec_2.tex <==
\section{Memorization vs Generalization}

Current approaches to language modeling rely on the memorization of infrequent words to perform well on generalization tasks \citep{feldman2020does}. Recent analytical work has shown that certain layers of transformer models implicitly encode frequency information \citep{kobayashi2023transformer}, while others store memorized long-tail data \citep{haviv2022understanding}.
\citet{feldman2020neural} demonstrate that models tend to memorize atypical examples as a result of implicit tuning for the highest accuracy on long-tailed data samples. This memorization hack, however, has only been shown to work well with over-parameterized models, when the number of weights surpasses the number of training samples \citep{belkin2019reconciling}. These findings suggest that with the current limited training objectives, generalization can only be achieved by large models trained on noisy datasets with sufficient long-tail samples \citep{Zheng2022AnES}.

\subsection{Representing Rare Tokens}
\citet{gao2018representation} showed that models trained as likelihood maximizers yield rare word embeddings that tend to cluster together in a degenerate manifold of the semantic space. Several diverse solutions have been proposed to deal with the problem. \citet{gong2018frage} introduces an adversarial training objective to push the embeddings of frequent and infrequent words to occupy a similar semantic space. \citet{gao2018representation} proposes a novel regularization term to the standard log-likelihood objective to better distribute the representation of rare words in semantic space. Other approaches have shown promising results on rare word performance by constructing token embeddings that take into account a word's surface form as well as surrounding context \citep{schick2019attentive,schick2020rare}. 

\subsection{Integrating Linguistic Information}
Before the widespread adoption of subword embeddings, researchers explored imbuing word embeddings with morphological and orthographic signals \citep{salle-villavicencio-2018-incorporating, vulic-etal-2017-morph, cotterell-schutze-2015-morphological, bhatia-etal-2016-morphological, both-blunsom-compositional-morphology}. Another line of related work proposes syntactically-motivated objective functions, such as predicting constituency labels \citep{wang2023language}, hypernyms \citep{bai-etal-2022-better}, dependency tags \citep{cui2022lert} and POS tags \citep{martinez-etal-2023-climb} to implicitly encode syntactic information in word representations.
